Robust Reinforcement Learning from Corrupted Human Feedback

Reinforcement learning from human feedback (RLHF) provides a principled framework for aligning AI systems with human preference data. For various reasons, e.g., personal bias, context ambiguity, lack of training, etc, human annotators may give incorrect or inconsistent preference labels. To tackle this challenge, we propose a robust RLHF approach -- $R^3M$, which models the potentially corrupted preference label as sparse outliers. Accordingly, we formulate the robust reward learning as an $\ell_1$-regularized maximum likelihood estimation problem. Computationally, we develop an efficient alternating optimization algorithm, which only incurs negligible computational overhead compared with the standard RLHF approach. Theoretically, we prove that under proper regularity conditions, $R^3M$ can consistently learn the underlying reward and identify outliers, provided that the number of outlier labels scales sublinearly with the preference sample size. Furthermore, we remark that $R^3M$ is versatile and can be extended to various preference optimization methods, including direct preference optimization (DPO). Our experiments on robotic control and natural language generation with large language models (LLMs) show that $R^3M$ improves robustness of the reward against several types of perturbations to the preference data.

==> theory.tex <==
%In this section, we prove that the reward function learned from corrupted data can be as accurate as its counterpart without outliers. To better convey our theoretical insights, we focus on the Markov decision process with horizon $m=1$, mirroring the setup in DPO (see Section \ref{sec:dpo}). Specifically, we consider learning the true reward function from the preference data of state-action pairs $\cD_{0}=\{(s_i, a_{1,i}, a_{2,i}, y_i)\}_{i=1}^N$, where $y_i = \ind(a_{1,i} \succ a_{2,i})$ denotes whether action $a_{1,i}$ is preferred to $a_{2,i}$. Notably, this setting finds extensive application in real-world scenarios. Take language models for instance. Our setting with horizon $m=1$ corresponds to comparing different responses to the same prompt, such as single-turn question-answering or text summarization task. To ease the theoretical analysis, we consider the tabular setting, where the number of states $|\cS|$ and the number of actions $|\cA|$ are finite. Here, we denote the true reward vector for the tabular case as $R^* = [r^*(s,a)]\in \RR^{|\cS||\cA|}$, with each entry $r^*(s,a)$ representing the true reward of some state-action pair, where $s\in\cS$ and $a\in\cA$.

We next establish the statistical guarantees for $R^3M$ on the reward recovery. Specifically, we prove that the reward function learned by $R^3M$ from corrupted human feedback can be as accurate as its counterpart without outliers. 

To better convey our theoretical insights, we consider a bandit setting, i.e., MDP with a horizon of one, mirroring the setup in DPO (see Section \ref{sec:dpo}). The preference data of state-action pairs are given as $\cD_{0}=\{(s_i, a_{1,i}, a_{2,i}, y_i)\}_{i=1}^N$, where $y_i = \ind(a_{1,i} \succ a_{2,i})$ denotes whether $a_{1,i}$ is preferred to $a_{2,i}$. Such a setting is common in real-world LLM applications such as (single-turn) question-answering or text summarization task, where $a_{1,i}$ and $a_{2,i}$ denote two different responses corresponding to the same prompt $s_i$.To ease the theoretical analysis, we consider a tabular setting, where the number of states $|\cS|$ and the number of actions $|\cA|$ are finite. For notational simplicity, we denote the true reward as a vector $R^* = [r^*(s,a)]\in \RR^{|\cS||\cA|}$, which concatenates the rewards of all state-action pairs, $r^*(s,a)$ with $s\in\cS$ and $a\in\cA$. %representing the true reward of some state-action pair, where $s\in\cS$ and $a\in\cA$.

Before we proceed with our main results, we first present the statistical guarantees of standard RLHF on the reward recovery, when there is no outlier in preference data ($\delta^* = 0$). Specifically, we can adapt Lemma 3.1 in \citet{zhu2023principled} to our setting: The Maximum Likelihood Estimator (MLE) $\hat{R}$ attains the following statistical rate of convergence: %converges to the true reward vector $R^*$ under the following rate:
\begin{equation}\label{eq:clean}
   \norm{\hat{R} - R^*}_{\Sigma_{0}}^2 = \cO\left(\frac{|\cS||\cA|}{n} \right),
\end{equation}
with overwhelming probability.
%where the notation $X_n = \cO_P(a_n)$ means that the set of v alues $X_n/a_n$ is bounded with high probability. 
Here, $\Sigma_{0} = \frac{1}{n} \sum_{i=1}^n  x_i x_i^\top$ is a positive semi-definite matrix depending on the training dataset $\cD_0$ with
$x_i = \ind(s = s_i, a=a_{1,i}) -  \ind(s = s_i, a=a_{2,i}) \in \RR^{|\cS||\cA|}$, and
$\left\|\cdot \right\|_{\Sigma_{0}}$ is the matrix norm defined as $\left\|v \right\|_{\Sigma_{0}}^2 = v^\top \Sigma_{0} v$ for any vector $v \in  \RR^{|\cS||\cA|}$.

\begin{remark} As has been shown in \citet{zhu2023principled}, given \eqref{eq:clean}, one can further prove the desirable regret bound for the learnt policy. Therefore, our theoretical analysis only focuses on the statistical guarantees on the reward recovery. %Our goal is to prove that learning the reward function in the existence of corrupted data can enjoy the same rate as that given in \eqref{eq:clean}.
\end{remark}

We then impose the following two assumptions on the problem.
\begin{assumption}\label{assump:sparse}
The perturbation $\delta^*$ only has $s\geq 0$ non-zero entries, i.e. $\|\delta^*\|_0 \leq s$. Moreover, there exists a constant $C >0$ such that $\|\delta^*\|_\infty \leq C$.
\end{assumption}
%Note that $s$ is allowed to scale with sample size $n$, while $C$ is not. %We remark that the sparse perturbation assumption is necessary, otherwise  the model is statistically unmanageable. 
%\zixuan{It seems to be repeated. Should we delete it?}
\begin{assumption}\label{assump:idt}
    Let $B>0$ be some constant. We have $r^* \in \cR_B$, where
    \begin{align*}
    \textstyle\cR_B = \left\{r :\cS \times\cA \to \RR~\big|~ \sum_{s \in \cS, a\in\cA} r(s,a) =0, \|R\|_2^2 = \sum_{s \in \cS, a\in\cA} (r(s,a))^2 \leq B\right\}.
    \end{align*}
\end{assumption}
Note that $s$ is allowed to scale with $(n,|S|,|A|)$, but $C$ and $B$ are not. This is mainly due to technical reasons to ensure the model identifiability. Accordingly, we adopt a constrained MLE formulation:
\begin{align}\label{eq:constrained-obj}
(\hat{r},\hat{\delta})=\argmin_{r,\delta} -\frac{1}{n}\sum_{i=1}^n\left [\log p(s_i,a_{1,i},a_{2,i},y_i;r,\delta)\right] + \lambda\|\delta\|_1\quad\textrm{subject~to}~r\in \cR_B,
\end{align}
where $p(s_i,a_{1,i},a_{2,i},y_i;r,\delta)$ is defined under the bandit setting as follows: 
\begin{align*}
p(s_i,a_{1,i},a_{2,i},y_i;r,\delta) = &\ind(y_i=1) 
     \sigma(r(s_i,a_{1,i})- r(s_i,a_{2,i}) + \delta_i) \\
     &+\ind(y_i=0) 
     \sigma(r(s_i,a_{2,i})- r(s_i,a_{1,i}) + \delta_i).
\end{align*}
Note that we add the constraint $r\in \cR_B$ in \eqref{eq:constrained-obj} also due to the technical reason under the tabular setting. In practice, the reward model with function approximation is usually trained with proper regularization, and therefore $r$ can be bounded without any constraint.
\begin{theorem}\label{thm}
    Suppose Assumptions \ref{assump:sparse} and \ref{assump:idt} hold. Let $\hat{R} = [\hat{r}(s,a)]$ and $\hat{\delta}$ be the minimizer of \eqref{eq:constrained-obj}. Given $\lambda = 1/n$, there exists universal constants $C_0>0$ and $\gamma$, such that we have
    \begin{align*}
        %\left\|\hat{R} - R^* \right\|_{\Sigma_{0}} \leq 
        \norm{\hat{R} - R^*}_{\Sigma_{0}}^2 + \frac{1}{n}\norm{\hat{\delta} - \delta^*}_2^2 \leq \frac{4}{\gamma^2} \left(\frac{4s}{n} + \frac{C_0|\cS||\cA|}{n}\right)
    \end{align*}
    with overwhelming probability. %Here   $\gamma = 1/(2+ \exp(-\sqrt{2}B-C) + \exp(\sqrt{2}B+C))$ . If we further set $\lambda = 1/n$, then with probability at least $1-\epsilon$,
    % \begin{align*}
    %     \left\|\hat{R} - R^* \right\|_{\Sigma_{0}} \leq \sqrt{\left\|\hat{R} - R^* \right\|_{\Sigma_{0}}^2 + \|\hat{\delta} - \delta^* \|^2 } \leq \frac{\sqrt{2}}{\gamma} \left( 2\sqrt{\frac{s}{n}} +C_1 \sqrt{\frac{|\cS||\cA| + \log(1/\epsilon)}{n} }\right).
    % \end{align*}
\end{theorem}
\begin{proof}[Proof Sketch] Due to space limit, we only present a proof sketch here. The technical proof of the lemmas can be found in Appendix \ref{sec:proof}. For notational simplicity, we denote $\Delta R = \hat{R} - R^*$ and $\Delta \delta = \hat{\delta} - \delta^*$, and denote the negative log-likelihood function on $\cD_0$ as
    \begin{align*}
        \cL(R,\delta) &=  -\frac{1}{n}\sum_{i=1}^n\left [\log p(s_i,a_{1,i},a_{2,i},y_i;r,\delta)\right] \\
        &= -\frac{1}{n}\sum_{i=1}^n\left[\log \left(\ind(y_i=1) 
     \sigma( \langle x_i, R \rangle + \delta_i) 
     +\ind(y_i=0) 
     \sigma( - \langle x_i, R \rangle + \delta_i)\right)\right] ,
    \end{align*}
    where we use $\langle x_i, R \rangle = \langle \ind(s = s_i, a=a_{1,i}) -  \ind(s = s_i, a=a_{2,i}), R\rangle = r(s_i,a_{1,i})- r(s_i,a_{2,i})$.
    Since $\hat{r} \in \cR_B$ and $\hat{\delta}$ are the minimizers of \eqref{eq:constrained-obj} and $r^* \in \cR_B$ by Assumption \ref{assump:idt}, we have
    \begin{equation}\label{eq:init}
        \cL(\hat{R}, \hat{\delta}) + \lambda\|\hat{\delta}\|_1 \leq \cL(R^*,\delta^*) + \lambda\|\delta^*\|_1.
    \end{equation}
The next Lemma proves the strong convexity of $\cL$ in $R$ and  $\delta$ at $(R^*, \delta^*)$ and $(\hat{R},\delta^*)$, respectively.
    \begin{lemma}\label{lemma:conv}
       Suppose Assumptions \ref{assump:sparse} and \ref{assump:idt} hold. Let $\gamma = 1/(2+ \exp(-\sqrt{2}B-C) + \exp(\sqrt{2}B+C))$.  $\cL$ is strong convex with respect to $R$ at $(R^*,\delta^*)$ with parameter $\gamma$,
    \begin{align}\label{convexity_R}
        \cL(R^*+ \Delta R,\delta^*) -  \cL(R^*,\delta^*) - \langle \nabla_R \cL(R^*,\delta^*), \Delta R \rangle \geq \gamma \|\Delta R \|_{\Sigma_{0}}^2.
    \end{align}
    Moreover, $\cL$ is $\gamma/n$-strong convex with respect to $\delta$ at $(\hat{R},\delta^*)$,
    \begin{align}\label{convexity_delta}
        \cL(\hat{R},\delta^*+\Delta \delta) -  \cL(\hat{R},\delta^*) - \langle \nabla_\delta \cL(\hat{R},\delta^*), \Delta \delta \rangle \geq \frac{\gamma}{n} \|\Delta \delta \|_2^2.
    \end{align}
    \end{lemma}
    Given the index set $\cS = \{i \in \{1,2,\ldots,n\} |\delta_i^* \neq 0 \}$ and $\cS^c = \{1,2,\ldots,n\}\setminus\cS$, we can decompose any $\delta \in \RR^n$ by the index set $\cS$ and $\cS^c $ as follows:
    \begin{equation*}
       \delta = \delta_\cS + \delta_{\cS^c}.
    \end{equation*}
    Here $\delta_\cS$ has the same non-zero entries as $\delta^*$. Now we apply the strong convexity of $\cL$ to \eqref{eq:init}, use Cauchy-Schwartz inequality to bound the inner product, and use decomposability of $\delta$ to obtain the following result.
    \begin{lemma}\label{lemma:itm1}
        Given the strong convexity of $\cL$ in \eqref{convexity_R} and \eqref{convexity_delta}, let $\lambda \geq \| \nabla_\delta\cL(\hat{R},\delta^*)\|_\infty$, we have
        \begin{align}\label{eq:itm1}
        \gamma \|\Delta R \|^2_{\Sigma_{0}} +\frac{\gamma}{n} \|\Delta \delta \|_2^2 \leq  2 \lambda \|\Delta \delta_\cS \|_1  +\|\nabla_R\cL(R^*,\delta^*) \|_{\Sigma_0^\dagger} \|\Delta R \|_{\Sigma_0}. 
    \end{align}
    \end{lemma}
    The above inequality suggests that we can control the estimation error of $\delta$ by only $\Delta \delta_\cS$, which can be regarded as the projection of $\Delta \delta$ onto the subspace $\{\delta \in \RR^n|\delta_j =0, \text{ for all } j \notin \cS \}$.
    The next lemma bounds the gradient of $\cL$ with respect to $\delta$:
     \begin{lemma}\label{lemma:grad-delta}
        For any $R \in \RR^{|\cS||\cA|}$ and $\delta \in \RR^n$, we have $\norm{\nabla_\delta \cL(\hat{R},\delta^*)}_\infty \leq 1/n$.
    \end{lemma}
    Therefore, it suffices to take $\lambda = 1/n$. Furthermore, in the proof of Lemma 3.1 of \citet{zhu2023principled} (See Section B.1 of \citet{zhu2023principled}), the gradient of $\cL$ with respect to $R$ can be bounded as following:
    \begin{lemma}\label{lemma:grad-R}
        There exists a universal constant $C_1>0$, such that we have
    \begin{align*}
        \|\nabla_R \cL(R^*,\delta^*) \|_{\Sigma_{0}^\dagger} \leq C_1 \sqrt{\frac{|\cS||\cA| + \log(1/\epsilon)}{n}}
    \end{align*}
 with probability at least $1-\epsilon$.
    \end{lemma}
    Finally, we combine Lemma \ref{lemma:itm1} and the upper bounds of gradients in Lemma \ref{lemma:grad-delta} and \ref{lemma:grad-R} to get
        \begin{align*}
        \|\Delta R \|^2_{\Sigma_{0}} +\frac{1}{n} \|\Delta \delta \|_2^2
        \leq \frac{4}{\gamma^2}  \left(  \frac{4s}{n} + C_1^2 \frac{|\cS||\cA| + \log(1/\epsilon)}{n} \right),
    \end{align*}
    which holds with probability at least $1-\epsilon$.
\end{proof}
We make the following remarks about Theorem \ref{thm}:


\begin{remark}
    When the data perturbation is sufficiently sparse, i.e. $s \leq |\cS||\cA|$, the convergence rate of estimating the reward under the presence of corrupted data is dominated by $|\cS||\cA|/n$. Notably, it is of the same order as that using clean data, which is presented in \eqref{eq:clean}. In other words, even there is contamination in data, the learned reward can still be as accurate as its counterpart without outliers.
%The condition of the sparse perturbation is necessary to achieve the fast convergence rate. 
However, if the ground-truth perturbation $\delta^*$ is not very sparse, i.e.  $s \gg |\cS||\cA|$, it can hurt the statistical rate of convergence.% as well as  make the problem statistically unmanageable \citep{wainwright2019high}.
\end{remark}
 

%\textbf{Moderate regularization:} The regularization parameter $\lambda$ for learning perturbation $\delta$ is required to be sufficiently small to learn the reward function efficiently. As suggested by Theorem \ref{thm}, it requires $\lambda = \cO(|\cS||\cA|/(\sqrt{s}n))$ to achieve the fastest convergence rate. Otherwise, high strength of regularization can impede the estimation of rewards.

\begin{remark}
    In our analysis, we estimate rewards for each state-action pair under the tabular bandit setting. However, our results can be extended to infinite-state and infinite-action case with reward function approximation, following \citet{zhu2023principled}. Specifically, our results work for the scenario where reward functions can be linearly approximated \citep{zhu2023principled}. Moreover, when the reward function is smooth, it can be approximated by neural networks and our analysis for convergence rate of reward recovery under corrupted preference data can apply as well 
    \citep{chen2020doubly}.
\end{remark}



